VoroCrust: Voronoi Meshing Without Clipping

Polyhedral meshes are increasingly becoming an attractive option with particular advantages over traditional meshes for certain applications. What has been missing is a robust polyhedral meshing algorithm that can handle broad classes of domains exhibiting arbitrarily curved boundaries and sharp features. In addition, the power of primal-dual mesh pairs, exemplified by Voronoi-Delaunay meshes, has been recognized as an important ingredient in numerous formulations. The VoroCrust algorithm is the first provably-correct algorithm for conforming polyhedral Voronoi meshing for non-convex and non-manifold domains with guarantees on the quality of both surface and volume elements. A robust refinement process estimates a suitable sizing field that enables the careful placement of Voronoi seeds across the surface circumventing the need for clipping and avoiding its many drawbacks. The algorithm has the flexibility of filling the interior by either structured or random samples, while preserving all sharp features in the output mesh. We demonstrate the capabilities of the algorithm on a variety of models and compare against state-of-the-art polyhedral meshing methods based on clipped Voronoi cells establishing the clear advantage of VoroCrust output.

==> tex/figs/sliver_fig.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}[b]{0.48\columnwidth}\centering
  \includegraphics[width=0.95\columnwidth,trim={17.25cm 13cm 18.5cm 11.25cm},clip]{figs/illustrations/sliver}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}\centering
  \includegraphics[width=0.95\columnwidth,trim={17.25cm 13cm 18.5cm 11.25cm},clip]{figs/illustrations/no_sliver}
\end{subfigure}
   \caption{Sliver elimination: (left) A quartet of balls centered at four samples (black) with four half-covered seeds yielding a Steiner vertex (pink) with four incident facets. (right) Shrinking resolves half-covered seeds and eliminates the Steiner vertex yielding only two facets. Refer to the supplemental materials for more details about this example.}
   \label{fig:slivers}
   \vspace{-6pt} 
\end{figure}


==> tex/tabs/vc_models_stat_tab.tex <==
\begin{table}[!tbh]
  \centering
	\setlength{\tabcolsep}{3pt}
	\resizebox{1.0\linewidth}{!}{
	\begin{tabular}{ccccccccc}
		\toprule
		Model & $Q_{min}$& $\theta_{<30}\%$& $\theta_{>90}\%$& $V_{6}\%$& $d_{H}(\times 10^{-2})$& $d_{RMS}(\times 10^{-3})$& $\rho_{min}$ &  \textit{Time} \\
		\cmidrule(rl){1-9}			
		 Bimba & 0.373 & 2 & 16 & 41 & 0.6142 & 0.782 & 0.187 & 935\\
		\hline
		Bird & 0.383 & 1 & 17 & 43 & 0.449 & 0.946 & 0.168 & 210\\		
		\hline
		Blade & 0.376 & 3 & 17 & 41 & 0.272 & 0.646 & 0.167 & 1584\\
		\hline		
		Bunny & 0.398 & 2 & 16 & 40 &  0.635 & 1.222 & 0.173 & 437\\
		\hline		
		Chinese Dragon & 0.358 & 2 & 16 & 40 & 0.332 & 0.588 & 0.171 & 3191\\		
		\hline		
		Close Spheres & 0.4 & 0.1 & 15 & 50 & 0.8506 & 2.392 & 0.205 & 4582\\
		\hline		
		David Head & 0.393 & 2 & 16 & 40 & 0.628 & 0.832 & 0.17 & 2697\\
		\hline
		Elephant & 0.375 & 2 & 16 & 42 & 0.755 & 0.839 & 0.123 & 2159\\		
		\hline		
		Fertility & 0.35 & 2 & 16 & 41 & 0.415 & 1.0 & 0.187 & 381\\		
		\hline		
		Femur & 0.414 & 2 & 16 & 42 & 0.334 & 0.892 & 0.189 & 42\\		
		\hline		
		Goat & 0.403 & 1 & 15 & 43 & 0.642 & 1.35 & 0.191 & 191\\		
		\hline		
		Hand & 0.432 & 2 & 16 & 42 & 1.018 & 1.016 & 0.197 & 130\\		
		\hline		
		Homer & 0.362 & 2 & 17 & 41 & 0.758 & 1.211 & 0.189 & 168\\		
		\hline		
		Loop & 0.383 & 2 & 16 & 41 & 0.171 & 0.271 & 0.185 & 1581\\		
		\hline		
		Omotondo & 0.356 & 2 & 17 & 41 & 0.509 & 0.659 & 0.195 & 2319\\		
		\hline		
		Spaghetti & 0.372 & 1 & 16 & 39 & 0.305 & 1.489 & 0.114 & 426\\		
		\hline		
		Noodles & 0.407 & 1 & 15 & 40 & 0.374 & 2.248 & 0.138 & 83\\		
		\hline		
		Rocker Arm & 0.38 & 2 & 16 & 39 & 0.486 & 0.526 & 0.175 & 96\\		
		\hline		
		Triceratops & 0.395 & 2 & 16 & 40 & 0.469 & 1.156 & 0.177 & 2136\\		
		\hline		
		Bracket & 0.15 & 20 & 24 & 33 & 0.215 & 0.34 & 0.092 &  43\\		
		\hline		
		Chazelle & 0.064 & 22 & 27 & 32 & 0.051 & 0.025 & 0.041 & 51\\		
		\hline		
		Complex Tube & 0.107 & 16 & 21 & 34 & 0.264 & 0.754 & 0.0462 & 1255\\		
		\hline		
		Two-hole Cylinder & 0.174 & 10 & 20 & 40 & 1.106 & 2.131 & 0.087 & 181\\		
		\hline		
		%Heptoroid & 0.273 & 11 & 20 & 35 & 0.087 & 0.124 & ? & 1464\\		
		%\hline		
		I-Beam & 0.221 & 14 & 22 & 33 & 0.202 & 0.205 & 0.061 & 2802\\		
		\hline		
		Joint & 0.149 & 19 & 23 & 32 & 0.569 & 0.643 & 0.08 & 32\\		
		\hline		
		Scorpion & 0.031 & 14 & 22 & 36 & 0.098 & 0.398 & 0.017 & 526\\		
		\hline		
		Two Boxes & 0.235 & 35 & 31 & 27 & 0 & 0 & 0.116 & 10\\		
		\hline		
		U-Part & 0.199 & 29 & 30 & 29 & 0.248 & 0.032 & 0.109 & 24\\		
		\hline
		Valve & 0.078 & 9 & 20 & 38 & 0.262 & 0.657 & 0.0381 & 380\\
		\bottomrule
	\end{tabular}
	}
	\caption*{ $Q_{min}$ is the minimum triangle quality. $\theta_{<30}\%$ and $\theta_{>90}\%$ are the percentage triangles with angle $< 30^{\circ}$ and $> 90^{\circ}$, respectively. $V_{6}\%$ is the percentage of surface mesh vertices with valence 6. $d_{RMS}$ is the root mean square distance and $d_{H}$ is Hausdorff distance normalized by the diameter of the bounding box. $\rho_{min}$ is the minimum Voronoi cell aspect ratio. \textit{Time} is the timing for generating surface spheres in seconds.}
	\label{tab:stat}
\end{table}
